Optimal Adaptive Experimental Design for Estimating Treatment Effect

Given n experiment subjects with potentially heterogeneous covariates and two possible treatments, namely active treatment and control, this paper addresses the fundamental question of determining the optimal accuracy in estimating the treatment effect. Furthermore, we propose an experimental design that approaches this optimal accuracy, giving a (non-asymptotic) answer to this fundamental yet still open question. The methodological contribution is listed as following. First, we establish an idealized optimal estimator with minimal variance as benchmark, and then demonstrate that adaptive experiment is necessary to achieve near-optimal estimation accuracy. Secondly, by incorporating the concept of doubly robust method into sequential experimental design, we frame the optimal estimation problem as an online bandit learning problem, bridging the two fields of statistical estimation and bandit learning. Using tools and ideas from both bandit algorithm design and adaptive statistical estimation, we propose a general low switching adaptive experiment framework, which could be a generic research paradigm for a wide range of adaptive experimental design. Through novel lower bound techniques for non-i.i.d. data, we demonstrate the optimality of our proposed experiment. Numerical result indicates that the estimation accuracy approaches optimal with as few as two or three policy updates.

==> figure/test.tex <==
\begin{figure}[htb]
\subfloat[Equilibrium Price]{
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
xmin=0, xmax=3.5,
ymin=0, ymax=2.3,
 axis x line=middle,
 xtick distance=1,
 ytick distance=.5,
legend pos=north west,
 axis y line=middle,
 x label style={at={(axis description cs:.5,-.1)},anchor=north},
  y label style={at={(axis description cs:-.1,.5)},rotate=90,anchor=south},
 xlabel=$\Delta$, ylabel=$p$,clip=false
]
\addplot+[name path=b1, mark=none, ultra thick, black] table [x=Delta, y=pI, col sep=comma]{data/laissez_faire_pI.csv};
\addlegendentry{$p_I^L$}
\addplot+[name path=b2, mark=none, thick, black, dashed] table [x=Delta, y =pE, col sep=comma]{data/laissez_faire_pE.csv};
\addlegendentry{$p_E^L$}
\addplot[only marks, mark=x, red, ultra thick]
    coordinates{ 
      (0.4512655218311157, 0)
    };
\addplot[only marks, mark=o, green, ultra thick]
    coordinates{ 
      (2.5000000000000000, 0)
    };
\addplot[only marks, mark=*, blue]
    coordinates{ 
      (3.0000000000000000, 0)
    };
\coordinate[label= {[yshift=-.7cm]$\Delta_1$} ] () at (0.45126, 0.3);
\coordinate[label= {[yshift=-.7cm]$\Delta_2$} ] () at (2.5, 0.3);
\coordinate[label= {[yshift=-.7cm]$\Delta_3$} ] () at (3.0, 0.3);
\end{axis}
\end{tikzpicture}}
\hfill
\subfloat[Equilibrium Demand]{
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
xmin=0, xmax=3.5,
ymin=0, ymax=2.3,
 axis x line=middle,
 xtick distance=1,
 ytick distance=.5,
legend pos=north west,
 axis y line=middle,
 x label style={at={(axis description cs:.5,-.1)},anchor=north},
  y label style={at={(axis description cs:-.1,.5)},rotate=90,anchor=south},
 xlabel=$\Delta$,ylabel=$q$,clip=false
]
\addplot+[name path=b1, mark=none, ultra thick, black] table [x=Delta, y=qI,col sep=comma]{data/laissez_faire_qI.csv};
\addlegendentry{$q_I^L$}
\addplot+[name path=b2, mark=none, thick, black, dashed] table [x=Delta, y=qE, col sep=comma]{data/laissez_faire_qE.csv};
\addlegendentry{$q_E^L$}
\addplot[only marks, mark=x, red, ultra thick]
    coordinates{ 
      (0.4512655218311157, 0)
    };
\addplot[only marks, mark=o, green, ultra thick]
    coordinates{ 
      (2.5000000000000000, 0)
    };
\addplot[only marks, mark=*, blue]
    coordinates{ 
      (3.0000000000000000, 0)
    };
\coordinate[label= {[yshift=-.7cm]$\Delta_1$} ] () at (0.45126, 0.3);
\coordinate[label= {[yshift=-.7cm]$\Delta_2$} ] () at (2.5, 0.3);
\coordinate[label= {[yshift=-.7cm]$\Delta_3$} ] () at (3.0, 0.3);
\end{axis}
\end{tikzpicture}}
\caption{(Color online) Equilibrium outcome under laissez-faire. We fix $v = 1.0, \gamma = 0.5$, and let $\Delta$ vary in $\mathbb{R}_+$. Notice that the threshold $\Delta_1$ would be defined later in Section~\ref{subsec: fair-reg}.}\label{fig: laissez-faire}
\end{figure}

==> old/note.tex <==
To do (Binary Numerical):
\begin{itemize}
    \item Base Model: $x \in \{L, H\}$, $y \in \{L, H\}, x \perp y$; $x$ can be disclosed; 
          $y$ can not be disclosed; pricing; compare disclose vs. non-disclose; 
          Single buyer.
          
    \item Extension 1: $y$ can also be disclosed -> three strategies.
    
    \item Extension 2: Multiple Seller. 
    $x$ can be disclosed (e.g., $(0,0), (1,1), (0,1)$ -> three strategy profiles; be aware of prisoner's dilemma); 
    If buyer pays search cost $c$, she knows \emph{both} sellers' $y$-realization -> advertising spillover effect; Buyer's demand (one unit or two units)?
    
    \item Extension 3: Multiple Buyer. 
          Participant engages in second-price auction.
    
    \item Note: Base and Extension 3 can be generalized to general distribution $f_1$, $f_2$.
\end{itemize}

==> old/package.tex <==
\usepackage{titling}
\usepackage{ae,aecompl}
\renewcommand{\familydefault}{\rmdefault}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
% \usepackage[latin9]{inputenc}
\usepackage[letterpaper]{geometry}
\geometry{verbose,tmargin=1in,bmargin=1in,lmargin=1in,rmargin=1in}
\usepackage{color}
\usepackage{babel}
\usepackage{float}
\usepackage{mathtools}
\usepackage{tcolorbox}
\usepackage{endnotes}
\makeatletter
%% Make a horizontal line below "Notes" 
% \def\enoteheading{\section*{\notesname
%   \@mkboth{\MakeUppercase{\notesname}}{\MakeUppercase{\notesname}}}%
%   \mbox{}\par\vskip-2.3\baselineskip\noindent\rule{.5\textwidth}{0.4pt}\par\vskip\baselineskip}
% \makeatother


% \PassOptionsToPackage{hyphens}{url}
% \usepackage{url}
% \PassOptionsToPackage{hyphens}{url}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage{esint}
\usepackage[authoryear]{natbib}
\onehalfspacing
% \usepackage[colorlinks=true,citecolor=blue,linkcolor=black,urlcolor=black]{hyperref}
\makeatletter
\newcommand{\noun}[1]{\textsc{#1}}
\providecommand{\tabularnewline}{\\}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{threeparttable}
\usepackage{multirow}
\theoremstyle{plain}
\usepackage{verbatim}
\providecommand{\tabularnewline}{\\}
\usepackage{enumerate}
\usepackage{comment}
\usepackage{mathpazo}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{observation}{Observation}
\newtheorem{condition}{Condition}
\usepackage{amsthm}
\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{example}{Example}\newtheorem{lemma}{Lemma}\newtheorem{proposition}{Proposition}\newtheorem{corollary}{Corollary}
% \newtheorem{problem}{Problem}
\newtheorem{instance}{Instance}
\usepackage{tikz}
\usepackage{eurosym}
\usepackage{caption}
\providecommand{\prop}{Proposition}
% \providecommand{\theoremname}{Theorem}
\usepackage{caption}
\usepackage{babel}
\PassOptionsToPackage{hyphens}{url}
\usepackage{hyperref}
\usepackage{appendix}
%\usepackage{scalerel,stackengine}
%\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
 \scaleto{%
 \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
 {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
 }{\textheight}% 
}{0.5ex}}%
\stackon[1pt]{#1}{\tmpbox}%
}
%\parskip 1ex
\def\spvec#1{\left(\vcenter{\halign{\hfil$##$\hfil\cr \spvecA#1;}}\right)}
\def\spvecA#1;{\if;#1;\else #1\cr \expandafter \spvecA \fi}
\usepackage{subfig}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepackage{pgfplotstable}
%\usetikzlibrary{arrows.meta,babel,calc,intersections,backgrounds,patterns,plotmarks,decorations.pathreplacing}
\usepackage{multirow}
%\usepgfplotslibrary{fillbetween}
\tikzstyle{every picture} += [>=stealth]
\makeatother
\usepackage{setspace}
\usepackage{lipsum}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Textclass specific LaTeX commands.
\newcommand{\new}[1]{\textcolor{red}{#1}}
\newcommand{\obs}[1]{\textcolor{gray}{#1}}
\newcommand*{\argmin}{\operatornamewithlimits{argmin}\limits}
\newcommand*{\argmax}{\operatornamewithlimits{argmax}\limits}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}%
\newcommand*{\QEDB}{\hfill\ensuremath{\square}}%

% code form: \pg{<the context>}
\newcommand{\ra}{\ensuremath{\rightarrow}} % abbreviation for right arrow
\newcommand{\PR}{\ensuremath{\mathsf{P}}} % probability
\newcommand{\E}{\ensuremath{\mathsf{E}}} % expectation
%\newcommand{\defeq}{\ensuremath{\triangleq}}
\newcommand{\subjectto}{\text{\textrm subject to}} % subject to
\renewcommand{\Re}{\ensuremath{\R}} % expectation
\newcommand{\bl}[1]{{\color{blue} {\sffamily\bfseries} #1}}
%%%%%%%% end of generic header

 \newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}
\newcommand*{\email}[1]{\texttt{#1}}
 \tikzset{
 hatch distance/.store in=\hatchdistance,
 hatch distance=10pt,
 hatch thickness/.store in=\hatchthickness,
 hatch thickness=2pt
 }
%\def\defeq{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}
 \makeatletter
 \pgfdeclarepatternformonly[\hatchdistance,\hatchthickness]{flexible hatch}
 {\pgfqpoint{0pt}{0pt}}
 {\pgfqpoint{\hatchdistance}{\hatchdistance}}
 {\pgfpoint{\hatchdistance-1pt}{\hatchdistance-1pt}}%
 {
 \pgfsetcolor{\tikz@pattern@color}
 \pgfsetlinewidth{\hatchthickness}
 \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
 \pgfpathlineto{\pgfqpoint{\hatchdistance}{\hatchdistance}}
% \PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
%  \usepackage{xurl}
 \pgfusepath{stroke}
 }
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\usetikzlibrary{shapes.geometric, arrows, calc, shapes.misc, matrix, shapes, arrows, calc, positioning, shapes.geometric, shapes.symbols, shapes.misc, intersections, chains, scopes}
\tikzstyle{node1} = [regular polygon, regular polygon sides=6,minimum width=1.25cm, text badly centered, text width=2.35em,minimum height=1.15cm, draw=black, font=\small]%,fill=red!40
\tikzstyle{node2} = [rectangle,rounded corners, minimum width=1.25cm, minimum height=4cm, text centered, draw=black, font=\small]%fill=orange!40,
\tikzstyle{arrow} = [thick,->,>=stealth]
 \tikzset{
 hatch distance/.store in=\hatchdistance,
 hatch distance=10pt,
 hatch thickness/.store in=\hatchthickness,
 hatch thickness=2pt
 }


\usepackage{tikz}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{hyperref}
\hypersetup{colorlinks=true,citecolor=blue}
\makeatother
% \usepackage{babel}
\usetikzlibrary{shapes.geometric, arrows, calc, shapes.misc, matrix, shapes, arrows, calc, positioning, shapes.geometric, shapes.symbols, shapes.misc, intersections, chains, scopes}
\tikzstyle{node1} = [regular polygon, regular polygon sides=6,minimum width=1.25cm, text badly centered, text width=2.35em,minimum height=1.15cm, draw=black, font=\small]%,fill=red!40
\tikzstyle{node2} = [rectangle,rounded corners, minimum width=1.25cm, minimum height=4cm, text centered, draw=black, font=\small]%fill=orange!40,
\tikzstyle{arrow} = [thick,->,>=stealth]
 \tikzset{
 hatch distance/.store in=\hatchdistance,
 hatch distance=10pt,
 hatch thickness/.store in=\hatchthickness,
 hatch thickness=2pt
 }
% \usepackage{mathtools}
\usepackage{mathtools}
\usepackage{setspace}
\usepackage{tikz}
\usetikzlibrary{arrows.meta, calc, fit, tikzmark}
\usepackage{mdframed}
\makeatletter

% \usepackage{ragged2e}
 
 \newcommand{\tikzmarks}[1]{\tikz[overlay,remember picture] \node (#1) {};}
 
 
\usepackage{array}
\renewcommand{\arraystretch}{1.5}
\makeatother
\newcommand{\pg}[1]{{\color{red} \noindent {Pin:} #1}}
\newcommand{\fxy}[2]{{\color{red} \noindent {Xingyu:} #2}}




\usepackage{algorithm}  
\usepackage{algorithmic}
\usepackage{setspace}
\usepackage{framed}
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother
\interfootnotelinepenalty=10000
\usepackage{apptools}
\usepackage{bbm}
\usepackage{chngcntr}
\usepackage{url}
\usepackage{setspace}
\usepackage{lipsum}
\makeatother
\usetikzlibrary{shapes.geometric, arrows, calc, shapes.misc, matrix, shapes, arrows, calc, positioning, shapes.geometric, shapes.symbols, shapes.misc, intersections, chains, scopes}
\tikzstyle{node1} = [regular polygon, regular polygon sides=6,minimum width=1.25cm, text badly centered, text width=2.35em,minimum height=1.15cm, draw=black, font=\small]%,fill=red!40
\tikzstyle{node2} = [rectangle,rounded corners, minimum width=1.25cm, minimum height=1cm, text centered, draw=black, font=\small]%fill=orange!40,
\tikzstyle{arrow} = [thick,->,>=stealth]
\onehalfspacing
\usepackage{clipboard}
\usepackage{hyperref}


==> old/proof_old1.tex <==
\paragraph{Uni-Attribute Product}
Say the focal firm chooses to provide a product with single attribute $z$ ($\delta_x = 0, \delta_y \in [0, 1]$). 
Then, the Gittins index of the un-searched uni-attribute product is denoted by $G_z$, which satisfies the following equation
\begin{align*}
    \mathbb{E}_{z} \Bigl[ \max\{0, z - p - G_z\} \Bigr] = 2c.
\end{align*}
Note that $G_z$ is exactly the reservation price defined in \cite{weitzman1979optimal}. 
To eliminate the trivial scenario, in which the consumer is unwilling to search the alternative $z$ even if it is free of charge and there is no outside option $u$, we assume the search cost is not too high, i.e., $c \in (0, \frac{1}{2})$, so that $G_z \geq 0$ when $p = 0$.
\begin{lemma}\label{lm: Gz}
The Gittins index of the un-searched uni-attribute product is given by
$$
G_z = 
\begin{cases}
1 - 4 c + \delta_z - p &\text{\quad, if $c \in (0, \frac{\delta_z}{2})$}\\
1 - 2 c - p &\text{\quad, if $c \in [\frac{\delta_z}{2}, \frac{1}{2}]$}
\end{cases}.
$$
\end{lemma}

%\begin{corollary}\label{cor: Gu}
% The Gittins index of the un-searched outside option is given by
% $$
% G_u = 2 - 4 c.
% $$
% \end{corollary}
% {\color{red}{$G_u$ seems to be very large. Maybe we can discard this in the base model.}}

We now intend to analyze its optimal pricing and design decisions. 
The firm's optimization problem is given by
\begin{align*}
     &\max_{p\geq 0, \delta_z \in [0, 1]} \quad  p \cdot \Bigl[ \frac{1}{2}\mathbb{I}\{1 - \delta_z - p \geq 0\} + \frac{1}{2}\mathbb{I}\{1 + \delta_z - p \geq 0\} \Bigr]\\
     &s.t. \qquad \qquad G_z \geq 0.
\end{align*}
\begin{proof}
We solve the problem stage-wise. The firm first pins down the product design $\delta_z$ and then decides the pricing $p$.
\begin{itemize}
    \item Case 1: If $\delta_z \in [0, 2c]$, then 
    $c \in [\frac{\delta_z}{2}, \frac{1}{2}]$. Clearly, $G_z = 1 - 2 c - p$. Then, the decision problem of the firm boils down to 
    \begin{align*}
     &\max_{p\geq 0, \delta_z \in [0, 2 c]} \quad p \cdot \Bigl[ \frac{1}{2}\mathbb{I}\{1 - \delta_z - p \geq 0\} + \frac{1}{2}\mathbb{I}\{1 + \delta_z - p \geq 0\} \Bigr]\\
     &s.t. \qquad \qquad p \leq 1 - 2 c.
\end{align*}
Note that because we have $p \leq 1 - 2 c$ and $0 \leq \delta_z \leq 2c$, then $p + \delta_z \leq 1$. Therefore, $1 + \delta_z - p \geq 1 - \delta_z - p \geq 0$ for sure. The optimal design is any $\delta_z^* \in [0, 2c]$ and price is $p^* = 1 - 2 c$, yielding revenue $1 - 2 c$.

    \item Case 2: If $\delta_z \in (2c ,1]$, then 
    $c \in (0, \frac{\delta_z}{2})$. Clearly, $G_z = 1 - 4 c + \delta_z - p$. 
    \begin{align*}
     &\max_{p\geq 0, \delta_z \in (2c ,1]} \quad p \cdot \Bigl[ \frac{1}{2}\mathbb{I}\{1 - \delta_z - p \geq 0\} + \frac{1}{2}\mathbb{I}\{1 + \delta_z - p \geq 0\} \Bigr]\\
     &s.t. \qquad \qquad   p \leq 1 - 4 c + \delta_z.
\end{align*}
    Note that $1 + \delta_z - p \geq 4 c > 0$. 
    
    If the firm chooses to abandon the low realization demand, namely, $1 - \delta_z - p < 0$, then $\delta_z^* = 1, p^* = 2 - 4c$, yielding revenue $\frac{2 - 4c}{2} = 1 - 2c$.
    
    If the firm preserves the low realization demand, namely, 
    $p \leq 1 - \delta_z$. Since $\delta_z > 2 c$, we have $1 - 4c + \delta_z > 1 - 4c + 2 c = 1 - 2c > 1 - \delta_z$. Thus, $\delta_z^* = 2 c, p^* = 1 - \delta_z^* = 1 - 2c$, yielding revenue $1 - 2c$.
    
    \item Now we compare Case 1 and Case 2. Clearly, the optimal revenue is $1 - 2 c$.
\end{itemize}
\end{proof}

==> old/proof_old2.tex <==
{\color{red}{Xingyu: Need some figures to vividly demonstrate the proof.}}

\paragraph{\underline{\underline{Proof of Proposition~\ref{prop: x_upper_bar}}}}
Define the left hand side of \eqref{def:search} as
\begin{align*}
    f(x) \triangleq \mathbb{E}_{y}\Bigl[ \max\{1 + x + y - p, 0\} \Bigr] = \int_{-\delta_y}^{+\delta_y} \frac{\max\{1 + x + y - p, 0\}}{2 \delta_y} d y.
\end{align*} 
To calculate $f(x)$, we have the following three cases:
\begin{itemize}
    \item When $x \in (-\infty, p - 1 - \delta_y)$, we have 
    $1 + x + y - p < 0, \forall y\in[-\delta_y, \delta_y].$
    Thus, we have $f(x) = \int_{-\delta_y}^{+\delta_y} \frac{\max\{1 + x + y - p, 0\}}{2 \delta_y} d y =  0$.
    
    \item When $x \in [p - 1 - \delta_y, p - 1 + \delta_y]$, we have $p - 1 - x \in [-\delta_y, \delta_y]$. Therefore, 
    \begin{align*}
        f(x) = \int_{-\delta_y}^{+\delta_y} \frac{\max\{1 + x + y - p, 0\}}{2 \delta_y} d y
        = \int_{p - 1 - x}^{+\delta_y} \frac{1 + x + y - p}{2 \delta_y} d y = 
        \frac{(1 + \delta_y - p + x)^2}{4 \delta_y}.
    \end{align*}
    
    \item When $x \in (p - 1 + \delta_y, +\infty)$, we have 
    $1 + x + y - p > 0, \forall y \in [-\delta_y, \delta_y].$ Hence, 
    $$
    f(x) = \int_{-\delta_y}^{+\delta_y} \frac{\max\{1 + x + y - p, 0\}}{2 \delta_y} d y = 
    \int_{-\delta_y}^{+\delta_y} \frac{1 + x + y - p}{2 \delta_y} d y = 1 - p + x.
    $$
\end{itemize}

The value of threshold $\overline{x}$ satisfies the following \textit{indifferent} condition
$$
    f(\overline{x}) = c,
$$
and we have the following two situations:
\begin{itemize}
    \item When $c \in (0, \delta_y]$, the straight line $c$ intersects with $f(x)$ at its second branch. Thus, we have
    \begin{align*}
        \frac{(1 + \delta_y - p + \overline{x})^2}{4 \delta_y} = c 
        \quad \Rightarrow \quad
        \overline{x} = p - 1 - \delta_y + 2\sqrt{\delta_y c}.
    \end{align*}
    
    \item When $c \in (\delta_y, +\infty)$, 
    the straight line $c$ intersects with $f(x)$ at its third branch. Therefore, we have
    \begin{align*}
        1 - p + \overline{x} = c 
        \quad \Rightarrow \quad 
        \overline{x} = c + p - 1.
    \end{align*}
\end{itemize}
\QEDA

\paragraph{\underline{\underline{Proof of Proposition~\ref{prop: pricing}}}}
Suppose the information design parameter $\delta$ has already been fixed. 
Now, we intend to optimize over product price $p$, given $\delta$ and $c$. 
We have the following cases:

\paragraph{\underline{Case I:} $c \geq 1 + \delta$.}
In this situation, we have 
$c \geq 1 + \delta \geq 1 - \delta = \delta_y$. Thus, by Proposition~\ref{prop: x_upper_bar}, we obtain the search threshold $\overline{x} = p + c - 1$. 
Furthermore, we have
$\overline{x} = p + c - 1 \geq c - 1 \geq \delta$, namely, even the most optimistic consumer will not initiate searching. 
Hence, the seller's optimal pricing strategy is to offer free product, resulting in zero profit, i.e., 
\begin{align*}
    p^*(\delta, c) =  0
    \quad , \quad
    \pi^*(\delta, c) = \pi\Bigl(p^*(\delta, c); \delta, c\Bigr) = 0.
\end{align*}

\paragraph{\underline{Case II:} $1 - \delta \leq c < 1 + \delta$.}
In this case, we have $c \geq 1 - \delta = \delta_y$, Thus, by Proposition~\ref{prop: x_upper_bar}, the search threshold is $\overline{x} = p + c - 1$. We have the following list of facts: 
\begin{itemize}
    \item $\overline{x} - (-\delta) = p + c - 1 + \delta \geq c - 1 + \delta \geq 0$. That is, the consumer with the ex-ante information $x \in [-\delta, \overline{x})$ will not search the product, and such region is non-empty.
    
    \item $1 + \overline{x} - (1-\delta) - p = c - 1 + \delta \geq 0$. 
    In other words, if the consumer has decided to search, she will always purchase the product even if her utility realization is in the worst scenario.
\end{itemize}
Combining the above two facts, the seller's profit function admits the following form
\begin{align*}
    \pi(p; \delta, c) 
    = \frac{\delta - \overline{x}}{2\delta} \cdot p 
    = \frac{\delta  + 1 - c - p}{2\delta} \cdot p.
\end{align*}
By first-order condition, we have 
\begin{align*}
    p^*(\delta, c) =  \frac{1 - c + \delta}{2}
    \quad , \quad
    \pi^*(\delta, c) = \pi\Bigl(p^*(\delta, c); \delta, c\Bigr) = \frac{(1 - c + \delta)^2}{8 \delta}.
\end{align*}

\paragraph{\underline{Case III:} $\delta \in [0, \frac{1}{2}] , 0 < c < \frac{-1+4 \delta-4 \delta^2}{-1+\delta}$.}
In this case, we have $c < \frac{-1+4 \delta-4 \delta^2}{-1+\delta} < 1 - \delta = \delta_y$. Thus, by Proposition~\ref{prop: x_upper_bar}, the search threshold becomes
$\overline{x} = p - 2 + \delta + 2\sqrt{(1 - \delta) c}$. 
Moreover, under the current parametric assumption, we can show the following inequality holds
\begin{align*}
    2 \delta < 2 - 2\delta - 2\sqrt{(1-\delta)c}.
\end{align*}

Now we study different pricing strategies:
\begin{itemize}
    \item When we choose $p \in [0, 2 \delta)$, then the search cut-off $\overline{x} \leq -\delta$, i.e., consumer always conducts active searching regardless of the ex-ante information $x$. 
    In addition, we have $1 + \delta - (1-\delta) - p \geq 0$. Therefore, the seller's profit function can be written as
    \begin{align*}
        \pi(p; \delta, c) = \frac{4\delta(1-\delta) - \frac{p^2}{2}}{4\delta(1-\delta)} \cdot p.
    \end{align*}
    \textit{If  $0< \delta < \frac{2}{5}$,} we can show the profit function is increasing in $p$, leading to 
    optimal price $2\delta$ and optimal profit
    $1 + \frac{1}{-1 + \delta} + 3 \delta$; 
    
    \textit{If $\frac{2}{5} \leq \delta <\frac{1}{2}$,} the profit function is concave with respect to $p$. By first-order condition, we have the optimal price 
    $2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$ and optimal profit $\frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$.
    
    \item When we choose $p \in [2 \delta, 2 - 2\delta - 2\sqrt{(1-\delta)c})$, then the search threshold $\overline{x} < -\delta$ while $1 + \delta - (1-\delta) - p < 0$. Thus, the seller's profit function admits the following form
    \begin{align*}
        \pi(p; \delta, c) = \frac{2\delta(1-\delta) - (p-\delta)\delta}{2\delta(1-\delta)} \cdot p.
    \end{align*}
    \textit{If $0 < \delta < \frac{2}{5}$,} then we can show $2\delta < 1 - \frac{\delta}{2}$, which is the stationary point of $\pi(p; \delta, c)$. 
    We have the following two sub-situations. \textit{if further $c > \frac{(2 - 3 \delta)^2}{16 (1 - \delta)}$,} then the pricing region $[2 \delta, 2 - 2\delta - 2\sqrt{(1-\delta)c})$ is at the left hand side of $\pi(p; \delta, c)$'s stationary point, which is $1 - \frac{\delta}{2}$. Thus, the optimal price is $2 - 2\delta - 2\sqrt{(1-\delta)c}$ and the optimal profit is $\frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 
   2 \sqrt{c - c \delta})}{-1 + \delta}$.
   \textit{If further $c \leq \frac{(2 - 3 \delta)^2}{16 (1 - \delta)}$,} then the pricing region contains $1 - \frac{\delta}{2}$. Thus, the optimal pricing is $1 - \frac{\delta}{2}$ and the result optimal profit is 
   $\frac{(-2 + \delta)^2}{8 (1 - \delta)}$;
    
    \textit{If $\frac{2}{5} \leq \delta < \frac{1}{2}$,} then the pricing region $[2 \delta, 2 - 2\delta - 2\sqrt{(1-\delta)c})$ is at the right hand side of $\pi(p; \delta, c)$'s stationary point, which is $1 - \frac{\delta}{2}$. Hence, 
    the optimal price is $2 \delta$ and the optimal profit is $1 + \frac{1}{-1 + \delta} + 3 \delta$.
    
    \item When we choose $p \in [2 - 2\delta - 2\sqrt{(1-\delta)c}, 2 - 2\sqrt{(1-\delta) c})$, then the search threshold $\overline{x}\in[-\delta, \delta]$, namely, only consumer receiving $x\in [\overline{x}, \delta]$ will conduct active search. We can write the seller's profit function as 
    \begin{align*}
        \pi(p; \delta, c) = 
        \frac{4 c (-1 + \delta) + (-2 + p)^2}{8 (1 - \delta) \delta} \cdot p.
    \end{align*}
    We can check the function $\pi(p; \delta, c)$ is deceasing in $p$. Thus, the optimal pricing is $2 - 2\delta - 2\sqrt{(1-\delta)c}$ and the resulted optimal profit is 
    $\frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{-1 + \delta}$.
    
    \item When we choose $p \in [2 - 2\sqrt{(1-\delta) c}, +\infty)$, 
    then the search cut-off $\overline{x} \geq \delta$. Thus, no consumer will conduct active search, resulting in zero seller's profit.
\end{itemize}

Now, we can proceed to compare the above four specific pricing strategies. There are three sub-cases:
\begin{itemize}
    \item[$\star$] When $\delta \in [\frac{2}{5}, \frac{1}{2}]$ and $c < \frac{-1+4 \delta-4 \delta^2}{-1+\delta}$, then the optimal profits under the above four pricing strategies are given by $\frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, $1 + \frac{1}{-1 + \delta} + 3 \delta$, 
    $\frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{-1 + \delta}$
    and $0$, respectively. 
    After careful examination, we have the first pricing scheme prevails, that is, 
    $$p^*(\delta, c)= 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}
    \quad,\quad 
    \pi^*(\delta, c) = \frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}.$$
    
    \item[$\star$] When $\delta \in [0, \frac{2}{5}]$ and $c < \frac{(2 - 3 \delta)^2}{16 (1 - \delta)}$, then the optimal profits under the above four pricing strategies are given by $1 + \frac{1}{-1 + \delta} + 3 \delta$, $\frac{(-2 + \delta)^2}{8 (1 - \delta)}$, $\frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{-1 + \delta}$ and $0$, respectively. 
    We can check that the second strategy dominates, namely, 
    \begin{align*}
        p^*(\delta, c) = 1 - \frac{\delta}{2}
        \quad,\quad 
        \pi^*(\delta, c) = \frac{(-2 + \delta)^2}{8 (1 - \delta)}.
    \end{align*}
    
    \item[$\star$] When $\delta \in [0, \frac{2}{5}]$ and $\frac{(2 - 3 \delta)^2}{16 (1 - \delta)} < c < \frac{-1+4 \delta-4 \delta^2}{-1+\delta}$, then the optimal profits under the above four pricing schemes are given by $1 + \frac{1}{-1 + \delta} + 3 \delta$, $\frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 
   2 \sqrt{c - c \delta})}{-1 + \delta}$, $\frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{-1 + \delta}$, and $0$, respectively. We can check that the second/third pricing strategy dominates, that is, 
   \begin{align*}
       p^*(\delta, c) = 2 - 2\delta - 2\sqrt{(1-\delta)c}
        \quad,\quad 
        \pi^*(\delta, c) = \frac{(-1 + \delta + \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{-1 + \delta}.
   \end{align*}
\end{itemize}

\paragraph{\underline{Case IV:} $\delta \in [0, \frac{1}{2}], \frac{-1 + 4 \delta - 4 \delta^2}{-1 + \delta} \leq c < 1 - \delta$.}
In this case, we have $c < 1 - \delta = \delta_y$. Thus, by Proposition~\ref{prop: x_upper_bar}, the search threshold becomes $\overline{x} = p - 2 + \delta + 2\sqrt{(1 - \delta) c}.$ 
Besides, in this parametric region, the following holds (reversing the comparison in Case III)
\begin{align*}
    2 - 2\delta - 2\sqrt{(1-\delta)c} < 2 \delta.
\end{align*}

Now we are ready to analyze the below four distinct pricing schemes:
\begin{itemize}
    \item When price $p \in [0, 2 - 2\delta - 2 \sqrt{(1 - \delta) c} )$, 
    then we have the search threshold $\overline{x} < -\delta$, that is, the consumer will always conduct active search regardless of her ex-ante information $x$. Besides, we have 
    $1 + \delta - (1 - \delta) - p = 2\delta - p \geq 0$. Thus, the seller's profit function can be formulated as
    \begin{align*}
        \pi(p; \delta, c) = \frac{4\delta(1-\delta) - \frac{p^2}{2}}{4\delta(1-\delta)} \cdot p.
    \end{align*}
    \textit{If $0 < \delta < \frac{2}{5}$,} then we can show the pricing region $[0, 2 - 2\delta - 2 \sqrt{(1 - \delta) c} )$ is always at the left hand side of the stationary point of $\pi(p; \delta, c)$, which is 
    $2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$. Hence, the function $\pi(p; \delta, c)$ is increasing in $p$. The optimal price is $2 - 2\delta - 2 \sqrt{(1 - \delta) c}$ and the resulted optimal profit is $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$.
    
    \textit{If $\frac{2}{5} < \delta < \frac{1}{2}$,} we have the following two sub-situations. 
    \textit{If further $c > 1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, }
    again, the function $\pi(p; \delta, c)$ is increasing in $p$. The optimal price is $2 - 2\delta - 2 \sqrt{(1 - \delta) c}$ and the resulted optimal profit is $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$. 
    \textit{If further $\frac{-1 + 4 \delta - 4 \delta^2}{-1 + \delta} < c < 1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$,} then the profit function is maximized at its stationary point. By first-order condition, the optimal price is 
    $2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$ and the corresponding optimal profit is 
    $\frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$. 
    
    
    \item When price $p \in [2 - 2\delta - 2 \sqrt{(1 - \delta) c}, 2\delta)$, then we have the search threshold $-\delta < \overline{x} < \delta$, i.e., only consumer receiving ex-ante information $x\in [\overline{x}, \delta]$ will actively search the product. Further note that $1 + \delta - (1 - \delta) - p = 2\delta - p \geq 0$. According to these facts, we can write the seller's profit as 
    \begin{align*}
        \pi(p; \delta, c) = 
        \frac{1 - c + \delta - p}{2 \delta} \cdot p.
    \end{align*}
    The stationary point of this profit function $\pi$ is at $p = \frac{1 - c + \delta}{2}$. Note that the stationary point satisfies
    $\frac{1 - c + \delta}{2} \leq 
    \frac{1 - \frac{-1 + 4 \delta - 4 \delta^2}{-1 + \delta} + \delta}{2} = \frac{\delta (-4 + 5 \delta)}{2 (-1 + \delta)} = 2\delta - \frac{\delta^2}{2 (1 - \delta)} < 2\delta$. We have the following two sub-situations. 
    
    \textit{If further $c > 5 - 3 \delta - 4 \sqrt{1 - \delta^2}$, } then the pricing interval contains the stationary point. Thus, the optimal price is $\frac{1 - c + \delta}{2}$, leading to optimal profit of size $\frac{(1 - c + \delta)^2}{8\delta}$.
    
    \textit{If further $\frac{-1 + 4 \delta - 4 \delta^2}{-1 + \delta} < c < 5 - 3 \delta - 4 \sqrt{1 - \delta^2}$, } the pricing range is at the right hand side of the stationary point. Namely, the profit function $\pi$ is decreasing in $p$, leading to optimal price $2 - 2\delta - 2 \sqrt{(1 - \delta) c}$ and the optimal corresponding optimal profit 
    $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$.
    
    \item When price $p \in [2\delta, 2 - 2\sqrt{(1-\delta) c})$, we have the search cut-off $\overline{x} \in (-\delta, \delta)$ and $1 + \delta - (1-\delta) - p = 2\delta - p \leq 0$. Thus, we can write the seller's profit as 
    \begin{align*}
        \pi(p; \delta, c) = 
        \frac{4 c (-1 + \delta) + (-2 + p)^2}{8 (1 - \delta) \delta} \cdot p .
    \end{align*}
    The stationary point of this function is at $p = -\frac{2}{3} (-2 + \sqrt{1 + 3 c - 3 c \delta})$. We can check $-\frac{2}{3} (-2 + \sqrt{1 + 3 c - 3 c \delta}) < 2\delta$ under the current parametric regime. 
    Therefore, the function is decreasing in $p$. Thus, the optimal price is $2\delta$, leading to the corresponding optimal profit of size $1 - c - \delta$.
    
    \item When price $p \in [2 - 2\sqrt{(1-\delta) c}, +\infty)$, we have the search cut-off $\overline{x} \geq \delta$. Thus, the optimal pricing strategy is to price at $0$ and the resulted profit is $0$.
\end{itemize}

Now, we are ready to pick the optimal pricing strategy. There are several sub-cases listed below:
\begin{itemize}
    \item[$\star$] When $\delta \in [0, \frac{1}{2}]$ and 
    $5-3 \delta-4 \sqrt{1-\delta^2} < c <1 - \delta$, the seller's profits under the four pricing strategies are given by 
    $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, $\frac{(1 - c + \delta)^2}{8\delta}$, $1 - c - \delta$, and $0$, respectively. Among these four strategies, we can show that the second one generates the highest profit, namely, 
    \begin{align*}
        p^*(\delta, c) = \frac{1 - c + \delta}{2}
        \quad, \quad
        \pi^*(\delta, c) = \frac{(1 - c + \delta)^2}{8\delta}.
    \end{align*}
    
    \item[$\star$] When $\delta \in [0, \frac{1}{2}]$ and 
    $\max\Bigl\{\frac{-1 + 4 \delta - 4 \delta^2}{-1 + \delta},  1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}\Bigr\} < c < 5-3 \delta-4 \sqrt{1-\delta^2}$, the profits under the four schemes are $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 2 \sqrt{c - c \delta})}{\delta}$,  $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, $1 - c - \delta$, and $0$, respectively. 
    We can show the first/second strategy yields the highest profit, that is, 
    \begin{align*}
        p^*(\delta, c) = 2 - 2\delta - 2 \sqrt{(1 - \delta) c}
        \quad, \quad
        \pi^*(\delta, c) = -\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 2 \sqrt{c - c \delta})}{\delta}.
    \end{align*}
    
    \item[$\star$] When $\delta \in [\frac{2}{5}, \frac{1}{2}]$ and $\frac{-1 + 4 \delta - 4 \delta^2}{-1 + \delta} < c < 1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, then the profits under the four pricing schemes are $\frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, $1 - c - \delta$, and $0$, respectively. After comparison, we find the first strategy yields the highest profit, i.e., 
    \begin{align*}
        p^*(\delta, c) = 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}
        \quad, \quad 
        \pi^*(\delta, c) = \frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}.
    \end{align*}
\end{itemize}

\paragraph{\underline{Case V:} $\delta \in [\frac{1}{2}, 1], c < 1-\delta$.}
In this case, we have $c < 1 - \delta = \delta_y$. Thus, by Proposition~\ref{prop: x_upper_bar}, the search threshold is $\overline{x} = p - 2 + \delta + 2\sqrt{(1 - \delta) c}.$ 
Besides, in this parametric range, we have the following holds
\begin{align*}
    2 - 2\delta - 2\sqrt{(1-\delta)c} 
    < 2 - 2\delta < 2\delta.
\end{align*}

Now we are ready to analyze the below four pricing schemes separately:
\begin{itemize}
    \item When price $p \in [0, 2-2\delta - 2 \sqrt{(1 - \delta) c} )$, 
    then we have the search threshold $\overline{x} < -\delta$, that is, the consumer will always conduct search regardless of her ex-ante information $x$. Besides, we have $1 + \delta -(1-\delta) - p =  2\delta - p > 0$. Therefore, the seller's profit function is
    \begin{align*}
        \pi(p; \delta, c) = \frac{4\delta(1-\delta) - \frac{p^2}{2}}{4\delta(1-\delta)} \cdot p.
    \end{align*}
    
    \textit{If $\delta \in [\frac{1}{2}, \frac{3}{5}]$, } we then have two sub-cases. \textit{If further $c > 1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, } then the profit function is increasing in $p$. Thus, the optimal price is $2-2\delta - 2 \sqrt{(1 - \delta) c}$, which leads to optimal profit of size 
    $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$. 
    \textit{If further $0< c < 1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$,} then the pricing interval contains the stationary point of $\pi$. Thus, the optimal price is $2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, which gives optimal profit of size $\frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$.
    
    \textit{If $\delta \in [\frac{3}{5}, 1]$, } then the profit function is increasing in $p$. Thus, the optimal price is $2-2\delta - 2 \sqrt{(1 - \delta) c}$, which leads to optimal profit of size 
    $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$.
    
    
    \item When price $p \in [2-2\delta - 2 \sqrt{(1 - \delta) c}, 2\delta)$, the profit function is 
    \begin{align*}
        \pi(p;\delta, c) = \frac{1 - c + \delta - p}{2 \delta} \cdot p. 
    \end{align*}
    The stationary point of the function $\pi$ is at $p = \frac{1 - c + \delta}{2}$. 
    Note that we  have $\frac{1 - c + \delta}{2} < \frac{1 + \delta}{2} < 2\delta$. 
    
    \textit{If $\delta \in [\frac{1}{2}, \frac{3}{5}]$, } then we have the following two sub-situations. \textit{If further $c > 5 - 3 \delta - 4 \sqrt{1 - \delta^2}$, } then the pricing interval contains the stationary point, that is, the optimal price is at $\frac{1 - c + \delta}{2}$ and the corresponding optimal profit is 
    $\frac{(1 - c + \delta)^2}{8 \delta}$.
    \textit{If further $0 < c < 5 - 3 \delta - 4 \sqrt{1 - \delta^2}$, } then the pricing interval is at the right hand side of the stationary point. Namely, the profit function is decreasing in $p$. Hence, the optimal price is at $2-2\delta - 2 \sqrt{(1 - \delta) c}$ and the optimal profit is $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$.
    
    \textit{If $\delta \in [\frac{3}{5}, 1]$, } then the pricing interval always contains the stationary point, that is, the optimal price is at $\frac{1 - c + \delta}{2}$ and the corresponding optimal profit is 
    $\frac{(1 - c + \delta)^2}{8 \delta}$.
    
    \item When price $p \in [2\delta, 2 - 2\sqrt{(1-\delta) c})$, then we can write the seller's objective function as 
    \begin{align*}
        \frac{4 c (-1 + \delta) + (-2 + p)^2}{8 (1 - \delta) \delta}  \cdot p.
    \end{align*}
    We can show the function is always decreasing in $p$. Hence, the optimal price is $2\delta$ and the resulted optimal profit is $1 - c - \delta$.
    
    \item When price $p \in [2 - 2\sqrt{(1-\delta) c}, +\infty)$, we have the search cut-off $\overline{x} \geq \delta$. 
    Thus, the optimal pricing strategy is to offer free product and the resulted profit is $0$.
\end{itemize}
We now compare the four pricing strategies. There are several situations.
\begin{itemize}
    \item[$\star$] When $\delta \in [\frac{1}{2}, \frac{3}{5}]$ and $5 - 3 \delta - 4 \sqrt{1 - \delta^2} < c < 1-\delta$, or, $\delta \in [\frac{3}{5}, 1]$ and $0 < c < 1-\delta$, then the profits under the four pricing schemes are 
    $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, $\frac{(1 - c + \delta)^2}{8 \delta}$, $1-c-\delta$, and $0$.
    We can show the second strategy is the optimal, that is, 
    \begin{align*}
        p^*(\delta, c) = \frac{1 - c + \delta}{2}
        \quad, \quad 
        \pi^*(\delta, c) = \frac{(1 - c + \delta)^2}{8 \delta}.
    \end{align*}
    
    
    \item[$\star$] When $\delta \in [\frac{1}{2}, \frac{3}{5}]$ and $1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta} < c < 5 - 3 \delta - 4 \sqrt{1 - \delta^2}$, then the profits under the four pricing schemes are given by $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, $1-c-\delta$, and $0$. 
    We can check the first/second strategy is optimal. That is, 
    \begin{align*}
        p^*(\delta, c) = 2-2\delta - 2 \sqrt{(1 - \delta) c}
        \quad , \quad
        \pi^*(\delta, c) = -\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}.
    \end{align*}
    
    
    \item[$\star$] When $\delta \in [\frac{1}{2}, \frac{3}{5}]$ and $0 < c < 1 - \frac{\delta}{3} - 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, then the profits under the four pricing schemes are 
    $\frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}$, $-\frac{(-1 + \delta + \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 
    2 \sqrt{c - c \delta})}{\delta}$, 
    $1 - c - \delta$, and $0$. We can check that the first strategy is optimal, namely,
    \begin{align*}
        p^*(\delta, c) = 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}
        \quad , \quad
        \pi^*(\delta, c) = \frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}.
    \end{align*}
\end{itemize}
\QEDA

\paragraph{\underline{\underline{Proof of Theorem~\ref{thm: info}}}}
For every given search cost $c > 0$, we intend to compute the seller's optimal information design choice $\delta^*(c)$, the resulted pricing decision $p^*(c) = p^*\Bigl(\delta = \delta^*(c) , c\Bigr)$, and the corresponding optimal profit $\pi^*(c) = \pi^*\Bigl(\delta = \delta^*(c) , c\Bigr)$. There are the following four cases:
\paragraph{\underline{Case I:} $c \in (0, \frac{1}{15})$.} 
We further have the below four information design strategies:
\begin{itemize}
    \item When $\delta \in (0, \frac{2}{5})$, then we have the equilibrium profit 
    $ 
        \pi^*(\delta, c) = \frac{(2 - \delta)^2}{8 (1 - \delta)}
    $
     and the corresponding pricing strategy is given by $
        p^*(\delta, c) = 1 - \frac{\delta}{2}
    $.
    Note that the function $\frac{(2 - \delta)^2}{8 (1 - \delta)}$ is increasing in $\delta$ when $\delta \in (0, \frac{2}{5})$. 
    Thus, the optimal information design choice is $\delta = \frac{2}{5}$ and the optimal pricing is $p = \frac{4}{5}$, which leads to profit of size $\pi = \frac{8}{15}$.
    
    \item When $\delta \in \Bigl(\frac{2}{5}, 
    -\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c]\Bigr)$, then we have the equilibrium profit
    $
    \pi^*(\delta, c) = \frac{4}{3} \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}
    $ and the corresponding pricing strategy is given by
    $
    p^*(\delta, c)= 2 \sqrt{\frac{2}{3}} \sqrt{(1 - \delta) \delta}
    $.
    We have the following two sub-situations.
    
    \textit{If further $c \in (0, \frac{5 - 2 \sqrt{6}}{6})$, } then we can check $\frac{1}{2} < -\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c]$. Thus, the information design region contains the stationary point of the profit function. Hence, the optimal design is $\delta = \frac{1}{2}$ and the optimal pricing is $p = \sqrt{\frac{2}{3}}$, which leads to optimal profit of size $\pi = \frac{2 \sqrt{\frac{2}{3}}}{3}$. 
    
    \textit{If further $c \in (\frac{5 - 2 \sqrt{6}}{6}, \frac{1}{15})$, } then we have 
    $\frac{1}{2} > -\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c]$, i.e., the profit function is increasing in $\delta$. Thus, the optimal information design is $\delta = -\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c]$ and the optimal pricing is $p = \frac{2}{25} \sqrt{2} \sqrt{(5 - 2 \sqrt{10 - 6 c} \sqrt{c} - c) \cdot (10 + 
    6 \sqrt{10 - 6 c} \sqrt{c} + 3 c)}$, which leads to optimal profit of size $\pi = \frac{4}{75} \sqrt{2} \sqrt{(5 - 2 \sqrt{10 - 6 c} \sqrt{c} - c) \cdot (10 + 
    6 \sqrt{10 - 6 c} \sqrt{c} + 3 c)}$.
    
    \item When $\delta \in \Bigl(-\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c], 
    \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}]\Bigr)$, then the equilibrium profit is 
    $
        \pi^*(\delta, c) = \frac{(1 - \delta - \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 2 \sqrt{c - c \delta})}{\delta}
    $ 
    and the pricing strategy is
    $
        p^*(\delta, c) = 2 - 2\delta - 2 \sqrt{(1 - \delta) c}
    $. 
    We have the following two sub-situations:
    
    \textit{If further $c \in (0, \frac{5 - 2 \sqrt{6}}{6})$, } we can check that the profit function is decreasing in $\delta$. Thus, the optimal information design is 
    $\delta = -\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c]$, the corresponding optimal pricing is $p = 
    \frac{2}{25} (10 + 6 \sqrt{10 - 6 c} \sqrt{c} + 3 c - 
   5 \sqrt{c (10 + 6 \sqrt{10 - 6 c} \sqrt{c} + 3 c)})$, and the resulted profit is 
   $\pi = \frac{2 (10 + 6 \sqrt{10 - 6 c} \sqrt{c} + 3 c - 
     5 \sqrt{c (10 + 6 \sqrt{10 - 6 c} \sqrt{c} + 3 c)})\cdot (9 \sqrt{
      10 - 6 c} \sqrt{c} + 17 c - 
     5 (2 + \sqrt{
        c (10 + 6 \sqrt{10 - 6 c} \sqrt{c} + 3 c)}))}{75 (-5 + 
     2 \sqrt{10 - 6 c} \sqrt{c} + c)}$.
    
    \textit{If further $c \in (\frac{5 - 2 \sqrt{6}}{6}, \frac{1}{15})$, } we can show that the stationary point of the profit function falls into the information design interval 
    $\Bigl(-\frac{3}{25} [-5 + 2 \sqrt{10 - 6 c} \sqrt{c} + c], 
    \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}]\Bigr)$.
    Thus, the optimal information design $\delta$ satisfies the following first-order condition
    \begin{align*}
        -6 c - 2 c^2 + (3 c + c^2) \delta + 2 \sqrt{c - c \delta} + 
  6 c \sqrt{c - c \delta} + \delta^2 (5 c - 6 \sqrt{c - c \delta}) = 0. 
    \end{align*}
    
    \item When $\delta \in \Bigl(\frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}], 1\Bigr)$, then the equilibrium profit is 
    $\pi^*(\delta, c) = \frac{(1 - c + \delta)^2}{8 \delta}$ and the equilibrium pricing is
    $p^*(\delta ,c) = \frac{1 - c + \delta}{2}$. We can show the optimal information design is $\delta = \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}]$ and the optimal pricing is 
    $p = \frac{2}{25} [10 - 7 c - \sqrt{(10 - c) c}]$, which leads to optimal profit of size 
    $\pi = \frac{2 (-10 + 7 c + \sqrt{(10 - c) c})^2}{
 25 (15 - 3 c - 4 \sqrt{(10 - c) c})}$.
\end{itemize}
We now can compare the above four information design strategies:
\begin{itemize}
    \item[$\star$] When $c \in (0, \frac{5 - 2 \sqrt{6}}{6})$, we can check the second informational scheme is optimal, that is, 
    \begin{align*}
        \delta^*(c) = \frac{1}{2}, \quad
        p^*(c) = \sqrt{\frac{2}{3}}, \quad
        \pi^*(c) = \frac{2\sqrt{\frac{2}{3}}}{3}.
    \end{align*}
    
    \item[$\star$] When $c \in (\frac{5 - 2 \sqrt{6}}{6}, \frac{1}{15})$, we can check the third informational scheme is optimal, that is, the optimal information design $\delta^*(c)$ satisfies the following first-order equation
    \begin{align*}
        -6 c - 2 c^2 + (3 c + c^2) \delta + 2 \sqrt{c - c \delta} + 
  6 c \sqrt{c - c \delta} + \delta^2 (5 c - 6 \sqrt{c - c \delta}) = 0,
    \end{align*}
    and the optimal pricing is
    $
        p^*(c) = 2 - 2\delta^*(c) - 2 \sqrt{(1 - \delta^*(c)) c}
    $,
    which leads to optimal profit of size
    $
        \pi^*(c) = \frac{(1 - \delta^*(c) - \sqrt{c - c \delta^*(c)}) \cdot (-1 - c + 3 \delta^*(c) + 2 \sqrt{c - c \delta^*(c)})}{\delta^*(c)}
    $. Denote such $\delta^*(c)$ as $\delta^*_1(c)$. By implicit function theorem, we can check $\delta^*_1(c)$ is decreasing in $c$.
\end{itemize}

\paragraph{\underline{Case II:} $c \in (\frac{1}{15}, \frac{1}{4})$.}
We have the following four informational schemes:
\begin{itemize}
    \item When $\delta \in (  0, \frac{2}{9} [3 - 4 c - 2 \sqrt{c (3 + 4 c)}]  )$, then we have 
    $
        p^*(\delta, c) = 1 - \frac{\delta}{2}
    $
    and
    $ 
        \pi^*(\delta, c) = \frac{(-2 + \delta)^2}{8 (1 - \delta)}
    $.
    We can check that the profit function is increasing in $\delta$. Thus, the optimal information design is $\delta = \frac{2}{9} [3 - 4 c - 2 \sqrt{c (3 + 4 c)}]$, and the optimal pricing is 
    $p = \frac{2}{9} (3 + 2 c + \sqrt{c (3 + 4 c)})$, which leads to optimal profit of size $\pi = \frac{2}{9} (3 + 5 c - 2 \sqrt{c (3 + 4 c)})$.
    
    
    \item When $\delta \in (  \frac{2}{9} [3 - 4 c - 2 \sqrt{c (3 + 4 c)}],  \frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}] )$, then $
       p^*(\delta, c) = 2 - 2\delta - 2\sqrt{(1-\delta)c}
    $
    and
    $
        \pi^*(\delta, c) = \frac{(1 - \delta - \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{1 - \delta}
   $.
   We have the following two sub-cases:
   
   \textit{If further $c \in (\frac{1}{15}, \sqrt{17}-4)$, } we can show the profit function is increasing in $\delta$. Thus, the optimal information design is $\delta = \frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}]$, which leads to optimal profit of size 
   $\pi = -\frac{1}{8 (4 + c + \sqrt{c} \sqrt{8 + c})} (-4 - c - \sqrt{c} \sqrt{8 + c} + 
    2 \sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})}) (4 - c - \sqrt{c} \sqrt{8 + c} + 
    4 \sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})})$.
   
   \textit{If further $c \in (\sqrt{17}-4, \frac{1}{4})$, } then the profit function is concave with respect to $\delta$. Thus, the optimal information design $\delta$ satisfies the following first-order equation
   \begin{align*}
       1 + \frac{(-4 + 3 \delta) \sqrt{c - c \delta}}{2 (1 - \delta)^2} = 0.
   \end{align*}
    
    \item When $\delta \in ( \frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}] ,  \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}] )$, then     $
        p^*(\delta, c) = 2 - 2\delta - 2 \sqrt{(1 - \delta) c}$ and
    $
        \pi^*(\delta, c) = \frac{(1 - \delta - \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 2 \sqrt{c - c \delta})}{\delta}
    $. We then have the following two-sub cases:
    
    \textit{If further $c \in (\frac{1}{15}, \sqrt{17}-4)$, } then we can show the profit function is concave with respect to $\delta$. Thus, the optimal information design $\delta$ satisfies the following first-order equation
    \begin{align*}
        -6 c - 2 c^2 + (3 c + c^2) \delta + 2 \sqrt{c - c \delta} + 
 6 c \sqrt{c - c \delta} + \delta^2 (5 c - 6 \sqrt{c - c \delta}) = 0.
    \end{align*}
    
    \textit{If further $c \in (\sqrt{17}-4, \frac{1}{4})$, } then we can check that the profit function is decreasing with respect to $\delta$. Thus, the optimal information design is $\delta = \frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}]$, which leads to optimal profit of size 
    $\pi = \frac{1}{8 (-4 + c + \sqrt{c} \sqrt{8 + c})} (-4 + 11 c + 
   3 \sqrt{c} \sqrt{8 + c} - 
   4\sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})}) (4 + c + 
   \sqrt{c} \sqrt{8 + c} - 
   2 \sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})})$.
    
    \item When $\delta \in (  \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}] ,  1 )$, then $p^*(\delta ,c) = \frac{1 - c + \delta}{2}$ and $\pi^*(\delta, c) = \frac{(1 - c + \delta)^2}{8 \delta}$. We can check the profit function admits the maximal value at information design $\delta = \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}]$, which leads to profit of size $\pi = 
    \frac{2 (-10 + 7 c + \sqrt{(10 - c) c})^2}{25 (15 - 3 c - 4 \sqrt{(10 - c) c})}$.
\end{itemize}
We are now ready to compare the above four informational schemes.
\begin{itemize}
    \item[$\star$] When $c \in (\frac{1}{15}, \sqrt{17}-4)$, the third informational strategy prevails. That is, the optimal information design $\delta^*(c) = \delta_1^*(c)$ satisfies:
    \begin{align*}
         -6 c - 2 c^2 + (3 c + c^2) \delta + 2 \sqrt{c - c \delta} + 
 6 c \sqrt{c - c \delta} + \delta^2 (5 c - 6 \sqrt{c - c \delta}) = 0,
    \end{align*}
    and 
    $
        p^*(c) = 2 - 2\delta^*(c) - 2 \sqrt{(1 - \delta^*(c)) c}
    $,
    $
        \pi^*(c) = \frac{(1 - \delta^*(c) - \sqrt{c - c \delta^*(c)}) \cdot (-1 - c + 3 \delta^*(c) + 2 \sqrt{c - c \delta^*(c)})}{\delta^*(c)}
    $. 
    
    \item[$\star$] When $c \in (\sqrt{17}-4, \frac{1}{4})$, the second strategy dominates. That is, the optimal information design $\delta^*(c)$ satisfies 
    \begin{align*}
        1 + \frac{(-4 + 3 \delta) \sqrt{c - c \delta}}{2 (1 - \delta)^2} = 0,
    \end{align*}
    and 
    $
       p^*(c) = 2 - 2\delta^*(c) - 2\sqrt{(1-\delta^*(c))c}
    $
    ,
    $
        \pi^*(c) = \frac{(1 - \delta^*(c) - \sqrt{c - c \delta^*(c)}) (\delta^*(c) + 2 \sqrt{c - c \delta^*(c)})}{1 - \delta^*(c)}
   $.
   Denote such $\delta^*(c)$ as $\delta_2^*(c)$. Utilizing the implicit function theorem, we can show $\delta_2^*(c)$ is decreasing in $c$.
\end{itemize}

\paragraph{\underline{Case III:} $c \in (\frac{1}{4}, 1)$.}
We further have the following three informational schemes:
\begin{itemize}
    \item When $\delta \in (0, 
    \frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}])$, then the equilibrium profit becomes 
    $
        \pi^*(\delta, c) = \frac{(1 - \delta - \sqrt{c - c \delta}) (\delta + 2 \sqrt{c - c \delta})}{1 - \delta}
   $, and the optimal pricing strategy is
    $
       p^*(\delta, c) = 2 - 2\delta - 2\sqrt{(1-\delta)c}
    $. 
    We can check that the profit function is decreasing in $\delta$ under the current parametric assumption. Therefore, the optimal information design is $\delta = 0$ and the optimal pricing is 
    $p = 2 - 2 \sqrt{c}$, leading to optimal profit of size $\pi = 2 \sqrt{c} - 2 c$.
    
    
    




    
    
    
    \item When $\delta \in (\frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}], \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}])$, then the equilibrium profit is 
    $
        \pi^*(\delta, c) = \frac{(1 - \delta - \sqrt{c - c \delta}) \cdot (-1 - c + 3 \delta + 2 \sqrt{c - c \delta})}{\delta}
    $,
    and the pricing strategy is
    $
        p^*(\delta, c) = 2 - 2\delta - 2 \sqrt{(1 - \delta) c}
    $.
    We can show the profit function is decreasing in $\delta$.
    Hence, the optimal information design is $\delta = \frac{1}{8} [4 - c - \sqrt{c} \sqrt{8 + c}]$ and the optimal pricing is $p = \frac{1}{4} (4 + c + \sqrt{c} \sqrt{8 + c} - 
   2 \sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})})$, which gives us the optimal profit of size 
   $
   \pi = \frac{1}{8 (-4 + c + \sqrt{c} \sqrt{8 + c})} (-4 + 11 c + 
   3 \sqrt{c} \sqrt{8 + c} - 
   4 \sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})}) \cdot (4 + c + 
   \sqrt{c} \sqrt{8 + c} - 
   2 \sqrt{2} \sqrt{c (4 + c + \sqrt{c} \sqrt{8 + c})})
   $.
    
    \item When $\delta \in \Bigl(\frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}], 1\Bigr)$, then the equilibrium profit is 
    $\pi^*(\delta, c) = \frac{(1 - c + \delta)^2}{8 \delta}$ and the equilibrium pricing is
    $p^*(\delta ,c) = \frac{1 - c + \delta}{2}$. We can show that the profit function is quasi-convex in $\delta$ when $\delta \in \Bigl(\frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}], 1\Bigr)$ and $c \in (\frac{1}{4}, 1)$. Therefore, the profit function is maximized at one of the two boundary points, that is, the maximal value is either $\pi^*\Bigl(\delta = \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}], c\Bigr) = 
    \frac{2 (-10 + 7 c + \sqrt{(10 - c) c})^2}{25 (15 - 3 c - 4 \sqrt{(10 - c) c})}$, 
    or, 
    $\pi^*\Bigl(\delta = 1, c\Bigr) = 
     \frac{(2 - c)^2}{8}$. We can show the two values satisfy single-crossing property. Specifically, we have the following two facts:
     
     \emph{If further $\frac{1}{4}< c < \frac{19 + \sqrt{161}}{50}$, } then  $\pi^*\Bigl(\delta = \frac{1}{25} [15 - 3 c - 4 \sqrt{(10 - c) c}], c\Bigr) = 
    \frac{2 (-10 + 7 c + \sqrt{(10 - c) c})^2}{25 (15 - 3 c - 4 \sqrt{(10 - c) c})}$ is the optimal profit. 
     
     \emph{If further $\frac{19 + \sqrt{161}}{50}<c<1$, } then $\pi^*\Bigl(\delta = 1, c\Bigr) = 
     \frac{(2 - c)^2}{8}$ is the optimal profit.
\end{itemize}

We can now check which informational scheme is optimal as $c$ varies in $(\frac{1}{4}, 1)$. 
It can be shown that the second informational scheme is dominated by the first one. Thus, we only need to compare the first and the third strategies. We can show when $c \in (\frac{1}{4}, \frac{19 + \sqrt{161}}{50})$, the third strategy is dominated by the first strategy. While, when $c \in (\frac{19 + \sqrt{161}}{50}, 1)$, there exists a unique threshold 
$\overline{c} \approx 0.815 \in (\frac{19 + \sqrt{161}}{50}, 1)$ satisfying
$
    2 \sqrt{\overline{c}} - 2 \overline{c} = \frac{(2 - \overline{c})^2}{8}.
$
To summarize, the equilibrium outcomes are given by below
\begin{itemize}
    \item[$\star$] When $c \in (\frac{1}{4}, \overline{c})$, we have
    \begin{align*}
        \delta^*(c) = 0, \quad 
        p^*(c) = 2 - 2\sqrt{c}, \quad 
        \pi^*(c) = 2\sqrt{c} - 2c.
    \end{align*}
    
    \item[$\star$] When $c \in (\overline{c}, 1)$, we have
    \begin{align*}
        \delta^*(c) = 1, \quad 
        p^*(\delta ,c) = 
        1 - \frac{c}{2}, \quad 
        \pi^*(c) = \frac{(2 - c)^2}{8}.
    \end{align*}
\end{itemize}

\paragraph{\underline{Case IV:} $c \in (1, 2)$.}
Then we have the following two information design strategies:
\begin{itemize}
    \item When $\delta \in (0, c - 1)$, then we have the equilibrium profit goes to zero.
    
    \item When $\delta \in (c - 1, 1)$, then the equilibrium profit is given by $\pi^*(\delta, c) = \frac{(1 - c + \delta)^2}{8 \delta}$ and the corresponding pricing strategy is $p^*(\delta ,c) = \frac{1 - c + \delta}{2}$. We can show the profit function $\frac{(1 - c + \delta)^2}{8 \delta}$ is increasing in $\delta$ under the current parametric assumption. Thus, the optimal information design is $1$ and the optimal pricing is $1 - \frac{c}{2}$, which leads to profit of size $\frac{(2 - c)^2}{8}$.
\end{itemize}
Clearly, we have the latter profit $\frac{(2 - c)^2}{8} \geq 0$. Thus, when $c \in (1, 2)$,
\begin{align*}
    \delta^*(c) = 1, \quad p^*(c) = 1 - \frac{c}{2}, \quad \pi^*(c) = \frac{(2 - c)^2}{8}.
\end{align*}

\noindent To summarize all the above four cases, we have 
$$
\delta^*(c) = 
\begin{cases}
\frac{1}{2} &\text{\quad , if $c \in (0, \frac{5-2\sqrt{6}}{6}]$}\\
\delta_1^*(c) &\text{\quad , if $c \in (\frac{5-2\sqrt{6}}{6}, \sqrt{17}-4]$}\\
\delta_2^*(c) &\text{\quad , if $c \in (\sqrt{17}-4, \frac{1}{4}]$}\\
0 &\text{\quad , if $c \in (\frac{1}{4}, \overline{c}]$}\\
1 &\text{\quad , if $c \in (\overline{c}, 2)$}
\end{cases}, 
p^*(c) = 
\begin{cases}
\sqrt{\frac{2}{3}} &\text{\quad , if $c \in (0, \frac{5-2\sqrt{6}}{6}]$}\\
2 - 2\delta_1^*(c) - 2 \sqrt{(1 - \delta_1^*(c)) c} &\text{\quad , if $c \in (\frac{5-2\sqrt{6}}{6}, \sqrt{17}-4]$}\\
2 - 2\delta_2^*(c) - 2\sqrt{(1-\delta_2^*(c))c} &\text{\quad , if $c \in (\sqrt{17}-4, \frac{1}{4}]$}\\
2-2\sqrt{c} &\text{\quad , if $c \in (\frac{1}{4}, \overline{c}]$}\\
1-\frac{c}{2} &\text{\quad , if $c \in (\overline{c}, 2)$}
\end{cases}.
$$
\QEDA

\paragraph{\underline{\underline{Proof of Proposition~\ref{prop: profit_surplus_welfare}}}}
We have already computed the equilibrium seller's profit at the proof of Theorem~\ref{thm: info}. What remains to be calculated is the equilibrium consumer surplus.

\paragraph{\underline{Case I:} $c \in (0, \frac{5 - 2\sqrt{6}}{6}]$.} We have the equilibrium information design $\delta^*(c) = \frac{1}{2}$ and price $p^*(c) = \sqrt{\frac{2}{3}}$. By Proposition~\ref{prop: x_upper_bar}, we can show that $\overline{x}^* = \sqrt{\frac{2}{3}} - \frac{3}{2} + \sqrt{2 c} \leq -\frac{1}{2}$ for sure, that is, every consumer will visit the offline costly channel but only those satisfying $1 + x + y - p^*(c) \geq 0$ will purchase. Therefore, the consumer surplus is calculated as follows:
\begin{align*}
    cs^*(c) 
    &= \int_{-\frac{1}{2}}^{-\frac{1}{2} + \sqrt{\frac{2}{3}}} \int_{-x + \sqrt{\frac{2}{3}} - 1}^{\frac{1}{2}} \Bigl[1 + x + y - \sqrt{\frac{2}{3}} - c\Bigr] dy dx + 
    \int_{-\frac{1}{2} + \sqrt{\frac{2}{3}}}^{\frac{1}{2}} \int_{-\frac{1}{2}}^{\frac{1}{2}} \Bigl[1 + x + y - \sqrt{\frac{2}{3}} - c\Bigr] dy dx - 
    c \cdot \frac{(\sqrt{\frac{2}{3}})^2}{2} \\
    &= 1 - \frac{8 \sqrt{\frac{2}{3}}}{9} - c.
\end{align*}

\paragraph{\underline{Case II:} $c \in (\frac{5 - 2\sqrt{6}}{6}, \sqrt{17} - 4]$.} The equilibrium information design is $\delta^*(c) = \delta_1^*(c)$ and price $p^*(c) = 2 - 2\delta_1^*(c) - 2 \sqrt{(1 - \delta_1^*(c)) c}$.

\paragraph{\underline{Case III:} $c \in (\sqrt{17} - 4, \frac{1}{4}]$.} 
The equilibrium information design is $\delta^*(c) = \delta_2^*(c)$ and the price is $p^*(c) = 2 - 2\delta_2^*(c) - 2\sqrt{(1-\delta_2^*(c))c}$.

\paragraph{\underline{Case IV:} $c \in (\frac{1}{4}, \overline{c}]$.} 
The equilibrium information design is $\delta^*(c) = 0$ and price is $p^*(c) = 2 - 2\sqrt{c}$. That is, the seller will remove all relevant information of the product from the online free channel. By Proposition~\ref{prop: x_upper_bar}, we have the search threshold be $\overline{x}^* = 0$, namely, every consumer will search. While, only the consumer with $y \geq p^*(c) - 1$ will purchase. Hence, the equilibrium consumer surplus is 
\begin{align*}
    cs^*(c) = \frac{1}{2}\int_{-1}^{p^*(c) - 1} \Bigl[-c\Bigr] d y + \frac{1}{2}\int_{p^*(c) - 1}^{1} \Bigl[ 1 + y - p^*(c) - c \Bigr] d y = 0.
\end{align*}

\paragraph{\underline{Case V:} $c \in (\overline{c}, 2)$.} 
The equilibrium information design is $\delta^*(c) = 1$ and price is $p^*(c) = 1 - \frac{c}{2}$. 
That is, the seller will fully disclose the information of the product via the free online channel. 
By Proposition~\ref{prop: x_upper_bar}, we have the search threshold $\overline{x}^* = p^*(c) - 1 + c =  \frac{c}{2}$. Besides, we have 
$1 + \overline{x}^* - p^*(c) = c > \overline{c} > 0$, that is, every searcher will purchase. Thus, the consumer surplus is calculated as follows
\begin{align*}
    cs^*(c) = \frac{1}{2}\int_{\overline{x}^*}^{1} \Bigl[1 + x - p^*(c) - c\Bigr] d x = \frac{(2 - c)^2}{16}.
\end{align*}
\QEDA
